A Learned Radiance-Field Representation for Complex Luminaires

We propose an efficient method for rendering complex luminaires using a high-quality octree-based representation of the luminaire emission. Complex luminaires are a particularly challenging problem in rendering, due to their caustic light paths inside the luminaire. We reduce the geometric complexity of luminaires by using a simple proxy geometry and encode the visually-complex emitted light field by using a neural radiance field. We tackle the multiple challenges of using NeRFs for representing luminaires, including their high dynamic range, high-frequency content and null-emission areas, by proposing a specialized loss function. For rendering, we distill our luminaires' NeRF into a Plenoctree, which we can be easily integrated into traditional rendering systems. Our approach allows for speed-ups of up to 2 orders of magnitude in scenes containing complex luminaires introducing minimal error.

==> Sections/3_Background.tex <==
\section{Background}
\subsection{Monte Carlo Direct Illumination}
\label{sec:2pathtracingandmitsuba}
The rendering equation~\cite{kajiya86} is the basis of all current realistic rendering techniques; it defines the total amount of energy emitted from a point in the scene along a particular viewing direction ${L}_o$ as a function of the incoming light ${L}_i$ and a bidirectional reflectance distribution function $f_r$ (BRDF) modeling the angular distribution of scattered light as
\begin{equation}
    \label{eq:rendereq}
    {L}_o(\px,\omega_o) = {L}_e(\px,\omega_o) + \int_\Omega{}f_r(\px,\omega_i,\omega_o)\,{L}_i(\px,\omega_i)(\omega_i\cdot \mathbf{n}_\px)d\omega_i,
\end{equation}
with ${L}_e(\px,\omega_o)$ the emission at $\px$, and $\mathbf{n}_\px$ the normal at $\px$. Note that the rendering equation is recursive, since $L_i$ is the result of the outgoing radiance at other point in the surface. 

Monte Carlo (MC) integration has dominated computer graphics ever since their introduction in ray tracing algorithms ~\cite{rlcook84}. Generally, MC methods stochastically estimate the expected value $F$ of a function $f(x)$ so that $F=\int f(x) \, dx$ by averaging a number $N$ of random samples, as
\begin{equation}
    F \approx \langle F \rangle = \frac{1}{N}\sum_{i=1}^N \frac{f(x_i)}{p(x_i)},
\end{equation}
with $\langle F \rangle$ the MC estimate of F, $x_i$ a random sample, and $p(x_i)$ the probability density function (pdf) of generating sample $x_i$. Monte Carlo methods are unbiased, and their error is solely characterized by the variance of the estimate. This variance vanishes as a rate of $O(N^{-\frac{1}{2}})$, and it is proportional to how well the probability function $p(x)$ fits $f(x)$. 

Thus, MC integration can be used to estimate radiance at every point of a scene. To compute $L_o(\px,\omega_o)$ we use the MC estimate defined as
\begin{equation}
L_o(\px,\omega_o) \approx \langle L_o(\px,\omega_o) \rangle = {L}_e(\px,\omega_o) + \frac{1}{N} \sum_{i=1}^N \frac{ f_r(\px,\omega_i,\omega_o)\,{L}_i(\px,\omega_i)(\omega_i\cdot \mathbf{n}_\px)}{p(\omega_i)},
\end{equation}
where $p(\omega_i)$ defines the probability of sampling the direction $\omega_i$. Thus, in order to maximize the variance reduction of the MC estimate, we would need to find a pdf such that $p(\omega_i)\propto f_r(\px,\omega_i,\omega_o)\,{L}_i(\px,\omega_i)(\omega_i\cdot \mathbf{n}_\px)$. However, sampling proportionally to the product of the BSDF and the incoming radiance is almost impossible for most scenarios. A more feasible approach would be to use two or more pdfs, proportional to each of the terms (e.g. $p(\omega_i)\propto\L_i(\omega_i))$, and combine them using some combination strategy (e.g. multiple importance sampling~\cite{veach97}). 


%MC methods are most efficient when, instead of uniformly sampling over the whole space, they proportionally sample the areas where radiance is higher, avoiding the potential waste of samples in areas where radiance is low. The basic aim of any importance sampling method is to place samples proportionally to the target distribution, so as to reduce variance and achieve better results with less samples. 
However, when light sources are occluded in most directions, or are hidden behind several layers of refractive materials, it is very hard to estimate where the actual light is coming from, and it is almost impossible to find a good $p(\omega_i)$. The reason is that the light incoming at $\px$ from direction $\omega_i$ is the result of potentially many bounces of high-frequency, difficult-to-sample, signals. Therefore, it is extremely unlikely to find a good sampling direction $\omega_i$, and the scene requires many samples to be rendered with low amounts of noise. This is exactly why rendering complex luminaires is so challenging: these luminaires contain many layers and small pieces of crystal, and even ornamental pieces of plastic, brass or cloth, that further scatter or block light in many directions. Thus, if we were to know in advance where the final radiance from the luminaire comes from we could implement efficient importance sampling techniques, leading to immense reductions of variance when rendering with low samples. %We believe our learned light field can be used in such a way; however, we leave this for future work.

\subsection{Neural Radiance Fields (NeRFs)}
\label{sec:nerf}
Neural Radiance Fields (NeRF) \cite{mildenhall2020} is a method for learning light fields of arbitrarily complex scenes from a set of sparse views and known camera poses, enabling the generation of views that were not contained in the original dataset. The essence of their approach can be summed in Figure \ref{fig:nerffigure}

\begin{figure}[!htbp]
   \begin{minipage}[b]{\columnwidth}
    \includegraphics[width=\columnwidth]{Figures/pipeline.jpg}
   \end{minipage}
   \caption[NeRF Pipeline]{NeRF pipeline overview. First, (a) it feeds positional and directional ray data to the model, which (b) uses an MLP to estimate color and density at a given location along the ray, and (c) volume rendering techniques to output a final color prediction. The MLP is then supervised by computing a (d) MSE rendering loss between the estimated and ground truth color. Image courtesy of ~\cite{mildenhall2020}}
   \label{fig:nerffigure}
\end{figure}

The key behind why NeRF performs so well when compared with previous methods lies in three main innovations:

\textit{Volume Rendering}. NeRF represents the scene's 5D radiance (light) field as the volume density and directional emitted radiance at any point in space. Consequentially, it uses traditional volume rendering techniques to estimate the color $\mathcal{C}(\Ray)$ of every ray $\Ray(t) = \px + t\,\omega$ traced across its volume as
\begin{equation}
    \label{eq:nerfequation}
    \mathcal{C}(\Ray) = \int_{t_n}^{t_f}\mathcal{T}(t)\,\sigma\left(\Ray(s)\right) \, c\left(\Ray(s), -\omega\right)\, dt, \text{ where } \mathcal{T}(t) = \exp\left(-\int_{t_n}^{t}\sigma\left(\Ray(s)\right)ds\right),
\end{equation}
with near and far bounds of the volume $t_n$ and $t_f$, respectively, and $\sigma\left(\px\right)$ and $c\left(\px, \omega\right)$ are the density and color at point $\px$ towards direction $\omega$, respectively. Finally, $\mathcal{T}(t)$ is the accumulated transmittance along the ray; once this value saturates, it means it has reached a surface in the scene, and its accumulated color along the ray is the resulting pixel value. Since volume rendering is differentiable, this allows them to learn the full 5D light field of the scene from only a set of views. 

\textit{Positional Encoding}. NeRF is able to learn high frequency functions thanks to its mapping of input coordinates (position and viewing direction) into a higher dimensional space using a set of periodic functions (Fourier features ~\cite{tancik2020fourfeat}). Given that networks are naturally biased towards learning lower frequency functions first ~\cite{mlbias}, by reformulating the input as a higher dimensional function they enable the network to learn higher frequency functions more easily. 

In essence, they map the three coordinate values in $\px$ and the three components of the Cartesian viewing direction unit vector $\omega$ into a higher dimensional space, from $\Real$ to $\Real^2\,L$, using a function $\gamma$ defined as
%
\begin{equation}
    \gamma(p) = (sin(2^0\pi{}p),cos(2^0\pi{}p),...,sin(2^{L-1}\pi{}p),cos(2^{L-1}\pi{}p)).
\end{equation}
The parameter $L$ is empirically set.

\textit{Coarse-to-fine Optimization}. NeRFs employ 2 different MLPs: a coarse model, and a fine model. This is done in order to avoid wasting a high amount of samples on empty space and occluded regions. The coarse model uses stratified sampling to sample a first set of $N_c$ locations along the ray, while the fine model uses this to make a more informed sampling, sampling a second set of $N_f$ locations on the most relevant parts of the volume, using a form of hierarchical sampling. 

More specifically, in order to bias the sample placement of the fine network towards the more relevant parts of the volume as detected by the coarse network, they rewrite the alpha composited color from the coarse network, as a weighted sum of all sampled colors $c_i$ along the ray
%
\begin{equation}
    \hat{\mathcal{C}_c}(r) = \sum_{i=1}^{N_c}w_i{}c_i \, ,\text{ where }  w_i = T_i(1-exp(-\sigma_i\delta_i))
\end{equation}
%
with $T_i$ being the transmittance until that point in the ray; essentially the cumulative sum of densities. If these weights are normalized, we obtain a piece-wise constant PDF along the ray. Now, sampling the second set of locations from this distribution can be performed by using inverse transform sampling, finally evaluating the fine network at the union between both sets of samples to compute the final rendered color of the ray. 


==> Sections/Anexo.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\@setckpt{Anexo\unhbox \voidb@x \penalty \@M \hskip \z@skip \unhbox \voidb@x \kern .06em\vbox {\hrule width.3em}\discretionary {-}{}{}\penalty \@M \hskip \z@skip SuppIndex}{
\setcounter{page}{25}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{46}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{AM@survey}{0}
\setcounter{parentequation}{0}
\setcounter{ContinuedFloat}{0}
\setcounter{Item}{0}
\setcounter{Hfootnote}{0}
\setcounter{bookmark@seq@number}{1}
\setcounter{section@level}{0}
}


==> Sections/Anexo_1.tex <==
\chapter{Project management, tools, other tests and further implementation details}
\label{an:annex1}
\section{Project management}
 Table \ref{table:management} shows a detailed breakdown of time spent in each section of the project.

\begin{table}[!htbp]
\begin{tabular}{|l|l|}
\hline
\textbf{Project Task}                                                                                                                                                      & \textbf{Estimated Time Spent} \\ \hline
\begin{tabular}[c]{@{}l@{}}Literature review: neural implicit geometry,\\ importance sampling, complex luminaires,\\ neural rendering, neural radiance fields\end{tabular} & 85h                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Datasets: modeling, generation and transformation\\ code\end{tabular}                                                                           & 50h                           \\ \hline
\begin{tabular}[c]{@{}l@{}}NeRF-SH: varied tests, HDR extension and \\significantly  expanded evaluation suite\end{tabular}                                                               & 350h                          \\ \hline
Ablation studies, model performance evaluations                                                                                                                            & 40h                           \\ \hline
NeRF-SH to Octree conversion                                                                                                                                               & 40h                          \\ \hline
Mitsuba NeRF expansion code                                                                                                                                                & 140h                          \\ \hline
Mitsuba tests                                                                                                                                                              & 60h                           \\ \hline
Thesis Document                                                                                                                                                            & 70h                           \\ \hline
\textbf{TOTAL}                                                                                                                                                             & \textbf{835h}                 \\ \hline
\end{tabular}
\caption[Project Management]{Project management}
\label{table:management}
\end{table}

\section{Tools}
Throughout this project I used the following tools:
\begin{enumerate}
    \item \textbf{Python}. General scripting, test development, and language used throughout most of the project.
    \item \textbf{C++}. Used in Mitsuba in order to extend its functionality.
    \item \textbf{Mitsuba}. Academic physically based renderer we extended for NeRF inference in our project.
    \item \textbf{JAX}. GPU Numpy and ML framework.
    \item \textbf{FLAX}. ML API for JAX.
    \item \textbf{Tensorflow}. We used its C API for model inference within Mitsuba.
    \item \textbf{Github}. Git tool used.
    \item \textbf{Pytorch}. NeRF-SH to Octree conversion.
    \item \textbf{WSL2}. Training and rendering in Linux within a Windows environment.
    \item \textbf{SSH}. Deploying workloads on the Lab workstations.
    \item \textbf{\LaTeX}. Writing this document.
\end{enumerate}

\section{Data generation}
In order to obtain an implicit representation of our luminaires, we first need some fine-quality renders. We modelled the different luminaires using Blender, using models and parts both original and taken from various sources \cite{cgtrader, turbosquid, 3ddd}. For the rendering part, we used Mitsuba. Mitsuba is an open-source, research-oriented rendering engine with plenty of features and parallelization in CPU. The fully accessible source code makes it suitable to our application, where we look to alter the how light sources are defined and queried inside Mitsuba. 

\subsection{Blender and Scene Composition}
We use Blender \cite{blender} to compose our luminaires. We designed a variety of different luminaires with different attributes to test our method. These attributes can be summed up in low-high frequency geometry, low-high frequency appearance, intensity of the specular highlights, dynamic range of the luminaire and low-high amounts of dark/non-emissive areas. In Section \ref{sc:datasets} we include an analysis of our selected scenes and their properties.  

In order to facilitate camera placement for the bulk generation of renders later on, the geometrical center of the luminaires was placed in the center of the scene. We used Blender 2.79 in order to take advantage of the Mitsuba scene exporter plugin. This plugin allows us to model our scenes in Blender and conveniently export the result into a Blender-style format, which uses a combination of .obj elements for the geometry and a HTML-style format for the scene description, which includes camera definition, geometry placement, light sources definition, material properties, etc. 

\subsection{Generation of the set of cameras}
Traditional NeRF, which is the base of our approach, fails when its cameras are placed at very different distances from the target geometry \cite{mipnerf}. More recent works, such as Mip-NeRF \cite{mipnerf}, account for this fact and enable a correct, anti-aliased representation of the target geometry at different distances and levels of detail, but it is not suitable to our application due to how rendering is carried out, using conical frustums instead of individual rays, which we need to be able to integrate properly into an overarching rendering engine. Therefore, we place all our cameras in a sphere surrounding our luminaire, at a distance which varies depending on the size of the luminaire. 

 It has been thoroughly demonstrated that NeRF representations fail when cameras are placed too far from each other, as the ability of the neural network to interpolate rapidly deteriorates~\cite{yu2020pixelnerf}. In order to avoid this issue, we generate camera positions using a Halton Low-Discrepancy Sequence, a pseudo-random number generation approach which is also used in path tracing samplers in rendering engines \cite{mitsuba}. Once we generate a 2D sequence of the required size (squared number of cameras), we geometrically warp it to the surface of a sphere, which yields the final unitary camera positions in XYZ coordinates. If required, we can scale them by any float number to account for luminaires of different sizes. %In Figure XXXX, we can observe some plots illustrating the 2D and 3D-warped samples and the notable differences between a fully random and a pseudo-random generation.

%Regarding the amount of cameras to generate, NeRF requires around a 100 images of the object being modelled in order to distill a high-quality representation; for this reason we sticked with a maximum of 100. We then generate between a 100 and 200 extra images for validation and testing purposes. %Given that our problem covers a full 360-degree sphere around the target geometry, we would probably need at least double that amount of images in order to obtain similar quality. In our testing, however, we observed how training times, which already are in the order of 3-4 days, would further extend when attempting to fit a larger number of images; for this reason we sticked with a maximum of 100. We then generate between a 100 and 200 extra images for validation and testing purposes.

\subsection{Rendering}
%As we already mentioned, we use Mitsuba 0.6, compiled for Linux, for rendering our luminaires. We selected Linux due to its easier compilation process and to the available hardware in the GiLab Workstation at our disposal.
In order to extend our testing capabilities during training and explore possible improvements to the network based on easily accessible ground truth data (given that our work full utilizes synthesized luminaires) we rendered 3 different representations of every luminaire: its appearance, stored as an HDR linear RGB image; its normal map; and its depth map (distance to the camera of every pixel in the luminaire. Every render carries its own alpha channel as well, and everything is stored as a multi-channel EXR file that we will later decompose into its different elements to adapt our dataset to the NeRF/NSVF dataset style and simplify our code. 

Rendering properties such as samples per pixel, integrator used, resolution, clipping planes distance and camera properties depended on the characteristics of each luminaire or the test objective of the dataset. In general, luminaires featuring volumetric components, such as tinted glasses, required a volumetric path tracer; while more difficult luminaires, featuring very small light sources, like single coils inside various layers of glass, required a bidirectional path tracer. Otherwise, we used a standard path tracer. Similarly, samples per pixel depended on luminaire complexity, while other camera characteristics were defined by luminaire size or other specific objectives of the dataset. 

Camera transformation matrix was computed using a look-at matrix scheme, which is easily defined by the generated XYZ positions in space of our cameras, an up vector (a constant vector 0,0,1) and a target XYZ position (fixed to 0,0,0)

In order to launch our complete set of renders at once and change the HTML scene file for each one to account for the varying camera positions, we use a Python interface to the Mitsuba rendering API integrated in Mitsuba 0.6.% Code and other minor details regarding this API can be seen in Annex \ref{an:annex2}.

Rendering was performed on a workstation featuring 2x Intel Xeon Gold (72 total threads), and rendering times varied drastically depending on the number of available threads at any given time, and luminaire complexity, but most datasets took around 2 or 3 days to generate. %In Figure XXX we can observe a sample of some of these renders for reference.

\subsection{Adapting to NeRF/NSVF dataset conventions}
Finally, we have our renders completed and we only need to adapt the dataset to the NeRF/NSVF format style. This allows us to recycle a good amount of code from the original NeRF implementation, which we later on expanded to accomodate all our changes. We implemented a Python script to separate the individual channels of our multi-channel EXR into RGB, normal and depth maps, generate the camera transformation matrices and store them in txt files, split between train, validation and test, normalize normal maps and depth maps, the latter using the near-far clipping plane distances used during rendering, and store each map, including both an EXR linear RGB map and PNG sRGB one, normal PNG and depth PNG into their own folders using the NSVF naming convention (files starting with 0\_{}, 1\_{}, and 2\_{} correspond to training, validation and test splits, respectively). 

\section{Other explored activation functions}
\subsection{Exponential activation function}
The most straightforward way of unbounding the RGB output was using an exponential activation function, going from (0,1) to (0,$\inf$). The function can be seen in Equation \ref{eq:exponential}. However, we found that in scenes where geometry had a large amount of black pixels, or exposed light sources with radiance peaks at specific values, the activation function was largely unstable. 

\begin{equation}
\label{eq:exponential}
    color = e^{x}
\end{equation}
\subsection{Softly-bounded log-sigmoid activation function}
In order to overcome the shortcomings of exponential activations, we tested with functions that would slightly bound the output. We did this by extending the range of the sigmoid function with a $log(x+1)$ function, which resulted in Equation \ref{eq:logsig}. One of the advantages of working with synthetic luminaires is that the maximum radiance that they output is known to us. By selecting the $\epsilon$ parameter, we could set the minimum and maximum range of our outputs: for example, for the \textit{portica} dataset, with a maximum radiance of ~12, we selected $\eps = 10^{-6}$, which results in an output range of $(10^{-6},13.8155)$. This activation function proved much more stable; however, it does not solve by itself the problem of extending to HDR: many of our luminaires have extreme dynamic ranges, and the most radiant areas in the luminaire dominate the error gradients, making an even learning of the radiance field difficult, with balance completely skewed towards exposed light sources and susceptible to high energy rendering noise. We further develop this issue when talking about our loss functions in Section \ref{ch:appearance:losses}.

\begin{equation}
\label{eq:logsig}
    color = -log(1 - \frac{1}{1+e^{-x}}+\epsilon)
\end{equation}

==> Sections/Anexo_2.tex <==
\chapter{Code}
\label{an:annex2}




==> Sections/Glossary.tex <==
\chapter*{Acronyms}
%each letter 12px
\textbf{MIS} \hspace{20px} Multiple Importance Sampling\\
\textbf{NeRF} \hspace{12px} Neural Radiance Field\\
\textbf{HDR} \hspace{12px} High Dynamic Range\\

